Automata and coalgebras in categories of species

We study generalized automata (in the sense of Ad\'amek-Trnkov\'a) in Joyal's category of (set-valued) combinatorial species, and as an important preliminary step, we study coalgebras for its derivative endofunctor $\partial$ and for the "Euler homogeneity operator" $L\circ\partial$ arising from the adjunction $L\dashv\partial\dashv R$. The theory is connected with, and in fact provides relatively nontrivial examples of, "differential 2-rigs", a notion recently introduced by the author putting combinatorial species on the same relation a generic (differential) semiring $(R,d)$ has with the (differential) semiring $\mathbb N[\![ X]\!]$ of power series with natural coefficients. The desire to study categories of "state machines" valued in an ambient monoidal category $(\mathcal K,\otimes)$ gives a pretext to further develop the abstract theory of differential 2-rigs, proving lifting theorems of a differential 2-rig structure from $(\mathcal R,\partial)$ to the category of $\partial$-algebras on objects of $\mathcal R$, and to categories of Mealy automata valued in $(\mathcal R,\otimes)$, as well as various constructions inspired by differential algebra such as jet spaces and modules of differential operators. These theorems adapt to various "species-like" categories such as coloured species, $k$-vector species (both used in operad theory), linear species (introduced by Leroux to study combinatorial differential equations), M\"obius species, and others.

==> fouche/alphabets.tex <==
\ExplSyntaxOn

\clist_new:N \g_fouche_upper_clist
\clist_gset:Nn \g_fouche_upper_clist { A,B,C,D,E,F,G,H,I,J,K,L,M,N,O,P,Q,R,S,T,U,V,W,X,Y,Z }

\clist_new:N \g_fouche_lower_clist
\clist_gset:Nn \g_fouche_lower_clist { a,b,c,d,e,f,g,h,i,j,k,l,m,n,o,p,q,r,s,t,u,v,w,x,y,z }

\clist_new:N \g_fouche_greek_clist
\clist_gset:Nn \g_fouche_greek_clist { alpha,beta,gamma,delta,epsilon,zeta,eta,theta,iota,kappa,lambda,mu,nu,xi,pi,rho, sigma,tau,upsilon,phi,chi,psi,omega,varphi,varpi,varepsilon,varrho,vartheta,Gamma,Delta,Theta,Lambda,Xi,Pi,Sigma,Upsilon,Phi,Chi,Psi,Omega }

\clist_new:N \g_fouche_both_clist
\clist_concat:NNN \g_fouche_both_clist \g_fouche_upper_clist \g_fouche_lower_clist

\clist_new:N \g_fouche_categories_clist
\clist_gset:Nn \g_fouche_categories_clist { Ab, Alg, Ban, BSD, Card, cat, Cat, Bij, CAT, cgHaus, Ch, CMnd, CMon, Comon, CW, Der, EM, End, Ext, Fin, fHilb, Fld, Foo, Fuk, fVect, Fzy, Gal, Grp, gVec, Nat, Haus, Het, Ho, Kl, Lat, Mag, coAlg, KSW, LAdj, Mac, Met, Mfd, Mnd, Mod, Mly, Mre, Acc, Mon, Ins, Ord, Par, PInj, POrd, Pos, Nom, PBij, Int, Pre, Pro, Prof, Quot, Quux, Rel, Ring, Rot, Set, Sgp, Sp, Spec, sSet, Sub, SW, Top, Tor, Inj, Unif, Vect, ArithCat, AbCat, SAbCat, Span, coSpan }

\clist_new:N \g_fouche_operators_clist
\clist_gset:Nn \g_fouche_operators_clist { lan, Lan, LAN, lft, Lft, LFT, ran, Hom, Ran, RAN, Rft, Yan, RFT, rft, op, co, coop, colim, coker, }

\cs_new_protected:Npn \fouche_makeabbrev:nnN #1 #2 #3
{
	\clist_map_inline:Nn { #3 }
	{
		\cs_new_protected:cpn { #2 } { #1 { ##1 } }
	}
}

\cs_new_protected:Npn \fouche_make_macro_abbrev:nnN #1 #2 #3
{
	\clist_map_inline:Nn { #3 }
	{
		\cs_new_protected:cpn { #2 } { #1 { \csname ##1\endcsname } }
	}
}

\fouche_makeabbrev:nnN { \textbf } { bf#1 } \g_fouche_both_clist
\fouche_makeabbrev:nnN { \boldsymbol } { bs#1 } \g_fouche_both_clist
\fouche_makeabbrev:nnN { \mathsf } { sf#1 } \g_fouche_both_clist
\fouche_makeabbrev:nnN { \mathfrak } { fk#1 } \g_fouche_both_clist
\fouche_makeabbrev:nnN { \underline } { un#1 } \g_fouche_both_clist

\fouche_makeabbrev:nnN { \mathcal } { cl#1 } \g_fouche_upper_clist
\fouche_makeabbrev:nnN { \mathbb } { bb#1 } \g_fouche_upper_clist

\fouche_makeabbrev:nnN { \mathsf } { #1 } \g_fouche_categories_clist
\fouche_makeabbrev:nnN { \mathrm } { #1 } \g_fouche_operators_clist

\DeclareMathAlphabet{\mybb}{U}{BOONDOX-ds}{m}{n}
\fouche_makeabbrev:nnN { \mybb } { mb#1 } \g_fouche_lower_clist

\fouche_make_macro_abbrev:nnN { \boldsymbol } { bs#1 } \g_fouche_greek_clist
\ExplSyntaxOff


==> fouche/envs.tex <==
\DeclareOption{english}{
	\theoremstyle{definition}
	\numberwithin{equation}{section}
	\newtheorem{theorem}{Theorem}[section]
	\defthm{corollary}{Corollary}
	\defthm{proposition}{Proposition}
	\defthm{lemma}{Lemma}
	\defthm{claim}{Claim}
	\defthm{question}{Question}
	\defthm{definition}{Definition}
	\defthm{notation}{Notation}
	\defthm{remark}{Remark}
	\defthm{conjecture}{Conjecture}
	\defthm{axiom}{Axiom}
	\defthm{example}{Example}
	\defthm{problem}{Problem}
	\defthm{examples}{Examples}
	\defthm{exercise}{Exercise}
	\defthm{counterexample}{Counterexample}
	\defthm{construction}{Construction}
	\defthm{warning}{Warning}
	\defthm{digression}{Digression}
	\defthm{perspective}{Perspective}
	\defthm{discussion}{Discussion}
	\defthm{terminology}{Terminology}
	\defthm{heuristics}{Heuristics}
	\defthm{conclusion}{Conclusion}
}

\makeatletter
\def\renewtheorem#1{%
	\expandafter\let\csname#1\endcsname\relax
	\expandafter\let\csname c@#1\endcsname\relax
	\gdef\renewtheorem@envname{#1}
	\renewtheorem@secpar
}
\def\renewtheorem@secpar{\@ifnextchar[{\renewtheorem@numberedlike}{\renewtheorem@nonumberedlike}}
\def\renewtheorem@numberedlike[#1]#2{\newtheorem{\renewtheorem@envname}[#1]{#2}}
\def\renewtheorem@nonumberedlike#1{
	\def\renewtheorem@caption{#1}
	\edef\renewtheorem@nowithin{\noexpand\newtheorem{\renewtheorem@envname}{\renewtheorem@caption}}
	\renewtheorem@thirdpar
}
\def\renewtheorem@thirdpar{\@ifnextchar[{\renewtheorem@within}{\renewtheorem@nowithin}}
\def\renewtheorem@within[#1]{\renewtheorem@nowithin[#1]}
\makeatother

\makeatletter
\def\redefthm#1#2{%
	\renewtheorem{#1}{#2}[section]%
	\expandafter\def\csname #1autorefname\endcsname{#2}%
	\expandafter\let\csname c@#1\endcsname\c@theorem}
\makeatother

\DeclareOption{italian}{
	\theoremstyle{definition}
	\numberwithin{equation}{section}
	\renewtheorem{theorem}{Teorema}[section]
	\redefthm{corollary}{Corollario}
	\redefthm{proposition}{Proposizione}
	\redefthm{lemma}{Lemma}
	\redefthm{definition}{Definizione}
	\redefthm{notation}{Notazione}
	\redefthm{remark}{Osservazione}
	\redefthm{conjecture}{Congettura}
	\redefthm{axiom}{Assioma}
	\redefthm{example}{Esempio}
	\redefthm{examples}{Esempi}
	\redefthm{exercise}{Esercizio}
	\redefthm{exercises}{Esercizi}
	\redefthm{counterexample}{Controesempio}
	\redefthm{construction}{Costruzione}
	\redefthm{warning}{Caveat}
	\redefthm{digression}{Digressione}
	\redefthm{perspective}{Prospettiva}
	\redefthm{discussion}{Discussione}
	\redefthm{terminology}{Terminologia}
	\redefthm{heuristics}{Euristica}
}

\DeclareDocumentEnvironment{enumtag}{m O{}}{%
	\begin{enumerate}[ label = \textsc{#1}\oldstylenums{\arabic*}), ref   = \textsc{#1}\oldstylenums{\arabic*}, #2] }{ \end{enumerate} }


==> fouche/macros.tex <==
\def\To{\Rightarrow}

\newcommand{\arXivPreprint}[1]{\href{http://arxiv.org/abs/#1}{arXiv:#1} preprint}

\newlength{\seplen}
\setlength{\seplen}{5pt}
\newlength{\sepwid}
\setlength{\sepwid}{.4pt}
\def\firstblank{\,\rule{\seplen}{\sepwid}\,}
\def\sndblank{\firstblank\llap{\raisebox{2pt}{\firstblank}}}

\newcommand{\celtag}[2][dr]{\ar[#1,white, "#2"{black,description}]}

\def\id{\text{id}}
\let\xto\xrightarrow
\let\xot\xleftarrow

\newcommand{\rot}[3][c]{\rotatebox[origin=#1]{#2}{$#3$}}
\newcommand{\rotarrow}[2][c]{\rot{#1}{#2}{\Rightarrow}}

\newcommand{\Nearrow}{\rotarrow{45}}
\newcommand{\Nwarrow}{\rotarrow{135}}
\newcommand{\Searrow}{\rotarrow{-45}}
\newcommand{\Swarrow}{\rotarrow{225}}
\newcommand{\Sarrow}{\rotarrow{-90}}
\newcommand{\Narrow}{\rotarrow{90}}

\newcommand{\bsmat}{\begin{smallmatrix}}
\newcommand{\esmat}{\end{smallmatrix}}

% \makeatletter
% \def\@cite#1#2{[\textsf{#1}\if@tempswa , #2\fi]}
% \def\@biblabel#1{[\textsf{#1}]}
% \makeatother
\def\cate#1{\mathsf{#1}}

\newcommand{\pto}{\mathop{\ooalign{\hfil\kern-2pt$\mapstochar$\hfil\cr\hfil$\longrightarrow$\hfil}}}

\usepackage{turnstile}
\newcommand{\adjunct}[2]{\nsststile{#2}{#1}}

\newcommand{\putbib}[2]{
	\bibliography{#1}{}
	\bibliographystyle{#2}
}

\usetikzlibrary{decorations.markings}
\tikzstyle{pro} =
[ decoration={ markings
		, mark = at position 0.5 with
			{\draw[-] (0,-1.25pt) -- (0,1.25pt);}
	}
, postaction ={decorate}
]

\newcommand*{\Scale}[2][4]{\scalebox{#1}{\ensuremath{#2}}}%
\def\lrc{
	\begin{tikzpicture}[scale=.33]
		\draw[-] (0,0) -| (1,1);
	\end{tikzpicture}
}
\makeatletter
\def\dopb{{\begin{tikzpicture}[scale=.375] \draw (0,0) -| (1,1);\end{tikzpicture}}}
\NewDocumentCommand{\xpb}{ O{dr} }{\ar@{}[#1]|(.375){\dopb}}
\def\dopo{{\begin{tikzpicture}[scale=.375] \draw (0,0) |- (1,1);\end{tikzpicture}}}
\NewDocumentCommand{\xpo}{ O{dr} }{\ar@{}[#1]|(.675){\dopo}}
\makeatother

\newcommand{\pb}{\arrow[dr, phantom, "\dopb", very near start]}
\newcommand{\po}{\arrow[dr, phantom, "\dopo", very near end]}

\def\[{\begin{equation}}
\def\]{\end{equation}}
% ^ this is BAD, but can't do without at this point...

\newenvironment{xsmallmatrix}[1]
{\renewcommand\thickspace{\kern#1}\smallmatrix}
{\endsmallmatrix}

\NewDocumentCommand{\prevar}{o m m}{
	\IfNoValueTF{#1}{
		\begin{smallmatrix}
			#2 \\
			\downarrow \\
			#3
		\end{smallmatrix}}
	{
		\begin{xsmallmatrix}{0em}
			& #2 \\
			#1 & \downarrow \\
			& #3
		\end{xsmallmatrix}}}

\ExplSyntaxOn
\NewDocumentCommand{\var}{o m O{s} m}{
	\str_case:nn { #3 } {
		{r}{\left(       \prevar[#1]{#2}{#4} \right)       }
		{s}{\left[       \prevar[#1]{#2}{#4} \right]       }
		{c}{\left\{      \prevar[#1]{#2}{#4} \right\}      }
		{a}{\left\langle \prevar[#1]{#2}{#4} \right\rangle }
	}}
\newcommand{\precop}[2]{
	\begin{smallmatrix}
		#1 \\ #2
	\end{smallmatrix}
}
\NewDocumentCommand{\cop}{O{r} m m}{
	\str_case:nn { #1 } {
		{r}{\left(       \precop{#2}{#3} \right)       }
		{s}{\left[       \precop{#2}{#3} \right]       }
		{c}{\left\{      \precop{#2}{#3} \right\}      }
		{a}{\left\langle \precop{#2}{#3} \right\rangle }
	}}

\NewDocumentCommand{\sm}{O{r} m}{
\str_case:nn { #1 } {
		{r}{\left(       \bsmat #2 \esmat \right)       }
		{s}{\left[       \bsmat #2 \esmat \right]       }
		{c}{\left\{      \bsmat #2 \esmat \right\}      }
		{a}{\left\langle \bsmat #2 \esmat \right\rangle }
	}
}
\ExplSyntaxOff

\usepackage{adjustbox}
\newenvironment{adju}[1][0.925]{%
	\begin{center}\begin{adjustbox}{max height=0.5\textheight, max width=#1\textwidth}}{\end{adjustbox}\end{center}}

\newenvironment{bareadju}[1][0.925]{%
	\begin{adjustbox}{max height=0.5\textheight, max width=#1\textwidth}}{\end{adjustbox}}


\def\emdash{\text{-}}
\NewDocumentCommand{\VCat}{ O{\clV} }{#1\emdash\Cat}
\def\twoCat{\VCat[2]}

\newcommand{\adja}[4]{
	#1 : \xymatrix{#2 \ar@<.5em>[r] \ar@{}[r]|\perp & \ar@<.5em>[l] #3 } : #4
}


\NewDocumentCommand{\vxy}{o m}{
	\IfNoValueTF{#1}
	{\vcenter{\xymatrix{#2}}} % do if \vxy{bla}
	{\vcenter{\xymatrix#1{#2}}} % do if \vxy[foo]{bla}
}

\newcommand{\de}{\partial}
\NewDocumentCommand{\FMly}{ O{} }{\IfNoValueTF{#1}{F\emdash\Mly}{F^{#1}\emdash\Mly}}
\NewDocumentCommand{\FMre}{ O{} }{\IfNoValueTF{#1}{F\emdash\Mre}{F^{#1}\emdash\Mre}}
\newcommand{\dMly}{\de\emdash\Mly}
\newcommand{\dMre}{\de\emdash\Mre}

\newcommand{\oo}[1]{#1^\op \times #1}

==> fouche/packages.tex <==

% \RequirePackage{amsthm}
\RequirePackage[svgnames]{xcolor}
\RequirePackage{ amsfonts
	, amsmath
	, amssymb
	, caption
	, epigraph
	, enumitem
	, lipsum
	, mathtools
	, hyphenat
	, tensor
	, todonotes
	, stackrel
	, tikz
	% , hyperref
	, savesym
	, setspace
	, tikz-cd
	, tcolorbox
	, booktabs
	, multirow
	, verbatim
	, calligra
	, url
}
\RequirePackage[all,2cell]{xy}\UseAllTwocells

% setup of specific packages

\usetikzlibrary{calc}
\usetikzlibrary{matrix,arrows}

\hypersetup{ bookmarksnumbered=true%
	, bookmarksopen=true%
	, breaklinks=true%
	, urlcolor=black%
	, colorlinks%
	, citecolor=black%
	, linkcolor=black%
	, urlcolor=black%
}

\tikzset{commutative diagrams/.cd,arrow style=tikz,diagrams={>=Straight Barb}}


==> fouche/page-layout.tex <==
%per le formule nei titoli
%-------------------------------------------------------------------------
\makeatletter
\g@addto@macro\bfseries{\boldmath}
\makeatother
%-------------------------------------------------------------------------

\makeatletter
\def\defthm#1#2{%
	\newtheorem{#1}{#2}[section]%
	\expandafter\def\csname #1autorefname\endcsname{#2}%
	\expandafter\let\csname c@#1\endcsname\c@theorem}
\makeatother

\tcbuselibrary{most}
\tcolorboxenvironment%
{quote}{ blanker
	, before skip=10pt
	, after skip=10pt
	, borderline west={6mm}{5pt}{gray!15}
	, breakable
}

\setcounter{tocdepth}{1}

